TexRO: Generating Delicate Textures of 3D Models by Recursive Optimization

This paper presents TexRO, a novel method for generating delicate textures of a known 3D mesh by optimizing its UV texture. The key contributions are two-fold. We propose an optimal viewpoint selection strategy, that finds the most miniature set of viewpoints covering all the faces of a mesh. Our viewpoint selection strategy guarantees the completeness of a generated result. We propose a recursive optimization pipeline that optimizes a UV texture at increasing resolutions, with an adaptive denoising method that re-uses existing textures for new texture generation. Through extensive experimentation, we demonstrate the superior performance of TexRO in terms of texture quality, detail preservation, visual consistency, and, notably runtime speed, outperforming other current methods. The broad applicability of TexRO is further confirmed through its successful use on diverse 3D models.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tabs/tab2_metric_shapenet.tex <==
\definecolor{tabfirst}{rgb}{1, 0.7, 0.7} % red
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7} % orange
\definecolor{tabthird}{rgb}{1, 1, 0.7} % yellow

\begin{table}
    \centering
    \begin{tabular}{l|ccc}
    & PSNR $\uparrow$ & LPIPS $\downarrow$ & Runtime \\ \hline

That 111one algorithm &  \cellcolor{tabthird}30.52 &  \cellcolor{tabthird}0.151 & 10 sec. \\
That other algorithm  & \cellcolor{tabsecond}32.13 & \cellcolor{tabsecond}0.074 & 100 sec. \\
Yet another algorithm &                      19.26 &                      0.433 & 3 sec. \\
\hline
My beloved algorithm  &  \cellcolor{tabfirst}38.92 &  \cellcolor{tabfirst}0.051 & 60 sec.

    \end{tabular}
    \caption{Wow what great results}
    \label{tab:results1}
\end{table}

==> tabs/tab3_controlnet_zero123.tex <==
\definecolor{tabfirst}{rgb}{1, 0.7, 0.7} % red
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7} % orange
\definecolor{tabthird}{rgb}{1, 1, 0.7} % yellow

\begin{table}
    \centering
    \begin{tabular}{l|cc}
    Method& FID $\downarrow$ & KID $\downarrow$ \\ \hline
Text2Tex~\cite{chen2023text2tex}&  \cellcolor{tabthird}34.14 &  \cellcolor{tabthird}5.94  \\
\hline
TexOpt+Zero123Plus&  \cellcolor{tabfirst}31.05 &  \cellcolor{tabfirst}4.86  \\
TexOpt+ControlNet  & \cellcolor{tabsecond}31.84 & \cellcolor{tabsecond}4.97 \\

    \end{tabular}
    \caption{Evaluation of different initialization methods in terms of FID and KID metrics. Our proposed multiview optimization is not significantly affected by the texture initialization model.}
    \label{tab:results2}
\end{table}

==> tabs/tab4_na.tex <==
\definecolor{tabfirst}{rgb}{1, 0.7, 0.7} % red
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7} % orange
\definecolor{tabthird}{rgb}{1, 1, 0.7} % yellow

\begin{table}
    \centering
    \begin{tabular}{l|cc}
    Method & FID $\downarrow$ & KID ($\times 10^{-3}$) $\downarrow$\\ \hline

Text2Tex~\cite{chen2023text2tex} & \cellcolor{tabthird}34.14 & \cellcolor{tabthird}5.94 \\
\hline 
TexOpt (w/o View Opt.)                    &  \cellcolor{tabsecond}32.75 &  \cellcolor{tabsecond}5.42 \\
TexOpt (w/ View Opt.)                    &  \cellcolor{tabfirst}31.05 &  \cellcolor{tabfirst}4.86
    \end{tabular}
    \caption{We further validate TexOpt on \texttt{Objaverse-Cap3D} with text prompts rich in semantics generated by Cap3D~\cite{luo2023scalable}. We also conduct an ablation on view optimization against using uniform views in this test.}
    \label{tab:objaverse_cap3d}
\end{table}

==> tabs/tab5_view_selection.tex <==
Optimal Viewpoints Selection\definecolor{tabfirst}{rgb}{1, 0.7, 0.7} % red
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7} % orange
\definecolor{tabthird}{rgb}{1, 1, 0.7} % yellow
\begin{table}[h]
    \centering
    \begin{tabular}{l|ccccc}
    & Step=5 &Step=13 & Step=20&Step=30 \\ \hline
FID&  35.00 & \cellcolor{tabfirst}31.05 & \cellcolor{tabsecond}31.55 & \cellcolor{tabthird}32.68 \\
KID  & 6.44 & \cellcolor{tabfirst}4.89 & \cellcolor{tabsecond}4.98 & \cellcolor{tabthird}5.49 & \\
    \end{tabular}
    \caption{The influence of selecting different denoising step counts on FID and KID metrics, demonstrating the feasibility of achieving favorable results for both metrics, particularly when utilizing a denoising step count of $13$.}
    \label{tab:results3}
\end{table}

==> tabs/tab6_time_comparision.tex <==
% \definecolor{tabfirst}{rgb}{1, 0.7, 0.7} % red
% \definecolor{tabsecond}{rgb}{1, 0.85, 0.7} % orange
% \definecolor{tabthird}{rgb}{1, 1, 0.7} % yellow

% \begin{table}
%     \centering
%     \begin{tabular}{l|ccc}
%     & PSNR $\uparrow$ & LPIPS $\downarrow$ & Runtime \\ \hline

% That 111one algorithm &  \cellcolor{tabthird}30.52 &  \cellcolor{tabthird}0.151 & 10 sec. \\
% That other algorithm  & \cellcolor{tabsecond}32.13 & \cellcolor{tabsecond}0.074 & 100 sec. \\
% Yet another algorithm &                      19.26 &                      0.433 & 3 sec. \\
% \hline
% My beloved algorithm  &  \cellcolor{tabfirst}38.92 &  \cellcolor{tabfirst}0.051 & 60 sec.

%     \end{tabular}
%     \caption{Wow what great results}
%     \label{tab:runtime}
% \end{table}
